AutoWeka4MCPS-AVATAR: Accelerating Automated Machine Learning Pipeline Composition and Optimisation

Automated machine learning pipeline (ML) composition and optimisation aim at automating the process of finding the most promising ML pipelines within allocated resources (i.e., time, CPU and memory). Existing methods, such as Bayesian-based and genetic-based optimisation, which are implemented in Auto-Weka, Auto-sklearn and TPOT, evaluate pipelines by executing them. Therefore, the pipeline composition and optimisation of these methods frequently require a tremendous amount of time that prevents them from exploring complex pipelines to find better predictive models. To further explore this research challenge, we have conducted experiments showing that many of the generated pipelines are invalid in the first place, and attempting to execute them is a waste of time and resources. To address this issue, we propose a novel method to evaluate the validity of ML pipelines, without their execution, using a surrogate model (AVATAR). The AVATAR generates a knowledge base by automatically learning the capabilities and effects of ML algorithms on datasets' characteristics. This knowledge base is used for a simplified mapping from an original ML pipeline to a surrogate model which is a Petri net based pipeline. Instead of executing the original ML pipeline to evaluate its validity, the AVATAR evaluates its surrogate model constructed by capabilities and effects of the ML pipeline components and input/output simplified mappings. Evaluating this surrogate model is less resource-intensive than the execution of the original pipeline. As a result, the AVATAR enables the pipeline composition and optimisation methods to evaluate more pipelines by quickly rejecting invalid pipelines. We integrate the AVATAR into the sequential model-based algorithm configuration (SMAC). Our experiments show that when SMAC employs AVATAR, it finds better solutions than on its own.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> algorithms/algorithm_bk.tex <==

\begin{algorithm}[htbp]
\scriptsize
\caption{Hybrid Pipeline Composition and Optimisation}
\begin{algorithmic}[1]

\Function{maximise} { $\mc{D}$, $\mc{A}$, $\mc{\lambda}$}

t <- newSearchTree()

\While{not satisfy stop condition}

\State{selectedNodes <- Selection(t,$\mc{D}$)}
\State{t <- ExpandSearchSpace(t, selectedNodes, $\mc{A}$)}
\State{t <- ReduceSearchSpace(t)}
\State{evaluatedPipelines <- PlayOut(t, $\mc{D}$)}
\State{bestPipeline <- BackPropagation(evaluatedPipelines)}

\EndWhile

\State{\textbf{return} bestPipeline }

\EndFunction

\\
\Function{Selection} {t,$\mc{D}$}

\State{selectedPipelines <- getTopPerformingPipeline($k_{\alpha}$, evalautedPipelines, qualityMetric)}
\State{selectedNodes <- getTopPerformingNode($k_\beta$, selectedPipelines, qualityMetric) }
\State{\textbf{return} selectedNodes}

\EndFunction



\\
\Function{ExpandSearchSpace} {t, selectedNodes, $\mc{A}$}

\State{t <- addNodesToLeafNodes(selectedNodes, $\mc{A}$)}

\State{\textbf{return} t}

\EndFunction

\\
\Function{ReduceSearchSpace} {t}

\For{leafNode in t}
    \State mlPipeline <- BackPropagation(leafNode,t,$\lambda=$default)
    \State \textbf{If} evaluateValidity(mlPipeline)$=$false \textbf{then} deactivate(leafNode)
    
\EndFor
      
\State{\textbf{return} y}

\EndFunction


\\
\Function{PlayOut} {t, $\mc{D}$}

\State population <- addPipelinesToPopulation(t, $k_{\gamma}$)
\State population <- performCrossOver(population)
\State population <- performMutation(mode=swapKPoints,population)
\State{\textbf{return} population}

\EndFunction



\\
\Function{BackPropagation} {t, leafNode, $\lambda$}

\State{p<- newMLPipeline()}

\While{true}
\State \textbf{If} $f_p$(leafNode)$!=$root 
\State \textbf{then} p <- append(p,$f_p$(leafNode))
\State \textbf{else} break 
\State
\EndWhile
\State{\textbf{return} p}
\EndFunction


\end{algorithmic}
\label{algorithm:hybrid_opt}
\end{algorithm} 

==> sections/exp_convergence_img.tex <==

\begin{landscape}

\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_abalone_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_abalone_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_abalone_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_abalone_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_abalone_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset abalone.}
    \label{fig:exp_convergence_abalone}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_adult_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_adult_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_adult_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_adult_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_adult_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset adult.}
    \label{fig:exp_convergence_adult}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_amazon_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_amazon_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_amazon_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_amazon_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_amazon_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset amazon.}
    \label{fig:exp_convergence_amazon}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_car_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_car_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_car_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_car_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_car_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset car.}
    \label{fig:exp_convergence_car}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_cifar10small_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_cifar10small_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_cifar10small_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_cifar10small_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_cifar10small_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset cifar10small.}
    \label{fig:exp_convergence_cifar10small}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_convex_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_convex_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_convex_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_convex_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_convex_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset convex.}
    \label{fig:exp_convergence_convex}
\end{figure*}






\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_dorothea_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_dorothea_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_dorothea_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_dorothea_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_dorothea_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset dorothea.}
    \label{fig:exp_convergence_dorothea}
\end{figure*}


\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gcredit_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gcredit_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gcredit_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gcredit_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gcredit_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset gcredit.}
    \label{fig:exp_convergence_gcredit}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gisette_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gisette_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gisette_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gisette_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_gisette_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset gisette.}
    \label{fig:exp_convergence_gisette}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_kddcup_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_kddcup_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_kddcup_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_kddcup_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_kddcup_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset kddcup.}
    \label{fig:exp_convergence_kddcup}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_krvskp_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_krvskp_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_krvskp_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_krvskp_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_krvskp_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset krvskp.}
    \label{fig:exp_convergence_krvskp}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_madelon_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_madelon_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_madelon_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_madelon_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_madelon_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset madelon.}
    \label{fig:exp_convergence_madelon}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_mnist_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_mnist_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_mnist_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_mnist_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_mnist_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset mnist.}
    \label{fig:exp_convergence_mnist}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_secom_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_secom_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_secom_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_secom_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_secom_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset secom.}
    \label{fig:exp_convergence_secom}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_semeion_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_semeion_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_semeion_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_semeion_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_semeion_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset semeion.}
    \label{fig:exp_convergence_semeion}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_shuttle_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_shuttle_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_shuttle_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_shuttle_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_shuttle_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset shuttle.}
    \label{fig:exp_convergence_shuttle}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_waveform_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_waveform_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_waveform_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_waveform_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_waveform_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset waveform.}
    \label{fig:exp_convergence_waveform}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_winequality_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_winequality_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_winequality_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_winequality_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_winequality_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset winequality.}
    \label{fig:exp_convergence_winequality}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_yeast_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_yeast_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_yeast_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_yeast_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/smac1/img_convergence_yeast_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of the dataset yeast.}
    \label{fig:exp_convergence_yeast}
\end{figure*}


\end{landscape}

==> sections/exp_convergence_img_smac1_merged30.tex <==



\begin{figure*}[h] 
   
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_abalone_seed0.pdf}
      }%
    %%\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_abalone_seed1.pdf}
        }%
    %%\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_abalone_seed2.pdf}
        }%
    %%\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_abalone_seed3.pdf}
        }%
    %%\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_abalone_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset abalone.}
    \label{fig:exp_convergence_smac1_abalone}
\end{figure*}











\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_amazon_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_amazon_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_amazon_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_amazon_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_amazon_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset amazon.}
    \label{fig:exp_convergence_smac1_amazon}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_car_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_car_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_car_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_car_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_car_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset car.}
    \label{fig:exp_convergence_smac1_car}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_cifar10small_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_cifar10small_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_cifar10small_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_cifar10small_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_cifar10small_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset cifar10small.}
    \label{fig:exp_convergence_smac1_cifar10small}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_convex_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_convex_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_convex_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_convex_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_convex_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset convex.}
    \label{fig:exp_convergence_smac1_convex}
\end{figure*}






\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_dorothea_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_dorothea_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_dorothea_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_dorothea_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_dorothea_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset dorothea.}
    \label{fig:exp_convergence_smac1_dorothea}
\end{figure*}


\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gcredit_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gcredit_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gcredit_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gcredit_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gcredit_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset gcredit.}
    \label{fig:exp_convergence_smac1_gcredit}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gisette_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gisette_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gisette_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gisette_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_gisette_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset gisette.}
    \label{fig:exp_convergence_smac1_gisette}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_kddcup_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_kddcup_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_kddcup_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_kddcup_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_kddcup_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset kddcup.}
    \label{fig:exp_convergence_smac1_kddcup}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_krvskp_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_krvskp_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_krvskp_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_krvskp_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_krvskp_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset krvskp.}
    \label{fig:exp_convergence_smac1_krvskp}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_madelon_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_madelon_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_madelon_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_madelon_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_madelon_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset madelon.}
    \label{fig:exp_convergence_smac1_madelon}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_mnist_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_mnist_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_mnist_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_mnist_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_mnist_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset mnist.}
    \label{fig:exp_convergence_smac1_mnist}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_secom_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_secom_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_secom_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_secom_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_secom_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset secom.}
    \label{fig:exp_convergence_smac1_secom}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_semeion_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_semeion_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_semeion_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_semeion_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_semeion_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset semeion.}
    \label{fig:exp_convergence_smac1_semeion}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_shuttle_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_shuttle_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_shuttle_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_shuttle_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_shuttle_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset shuttle.}
    \label{fig:exp_convergence_smac1_shuttle}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_waveform_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_waveform_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_waveform_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_waveform_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_waveform_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset waveform.}
    \label{fig:exp_convergence_smac1_waveform}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_winequality_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_winequality_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_winequality_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_winequality_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_winequality_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset winequality.}
    \label{fig:exp_convergence_smac1_winequality}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac1_merged/img_convergence_smac1_merged_yeast_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_yeast_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_yeast_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_yeast_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac1_merged/img_convergence_smac1_merged_yeast_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with (solid line) and without (dash line) the AVATAR using the dataset yeast.}
    \label{fig:exp_convergence_smac1_yeast}
\end{figure*}




==> sections/exp_convergence_img_smac5.tex <==

\begin{landscape}

\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_abalone_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_abalone_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_abalone_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_abalone_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_abalone_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset abalone.}
    \label{fig:exp_convergence_smac5_abalone}
\end{figure*}











\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_amazon_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_amazon_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_amazon_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_amazon_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_amazon_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset amazon.}
    \label{fig:exp_convergence_smac5_amazon}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_car_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_car_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_car_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_car_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_car_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset car.}
    \label{fig:exp_convergence_smac5_car}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_cifar10small_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_cifar10small_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_cifar10small_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_cifar10small_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_cifar10small_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset cifar10small.}
    \label{fig:exp_convergence_smac5_cifar10small}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_convex_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_convex_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_convex_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_convex_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_convex_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset convex.}
    \label{fig:exp_convergence_smac5_convex}
\end{figure*}






\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_dorothea_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_dorothea_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_dorothea_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_dorothea_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_dorothea_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset dorothea.}
    \label{fig:exp_convergence_smac5_dorothea}
\end{figure*}


\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gcredit_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gcredit_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gcredit_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gcredit_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gcredit_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset gcredit.}
    \label{fig:exp_convergence_smac5_gcredit}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gisette_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gisette_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gisette_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gisette_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_gisette_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset gisette.}
    \label{fig:exp_convergence_smac5_gisette}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_kddcup_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_kddcup_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_kddcup_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_kddcup_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_kddcup_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset kddcup.}
    \label{fig:exp_convergence_smac5_kddcup}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_krvskp_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_krvskp_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_krvskp_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_krvskp_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_krvskp_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset krvskp.}
    \label{fig:exp_convergence_smac5_krvskp}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_madelon_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_madelon_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_madelon_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_madelon_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_madelon_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset madelon.}
    \label{fig:exp_convergence_smac5_madelon}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_mnist_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_mnist_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_mnist_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_mnist_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_mnist_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset mnist.}
    \label{fig:exp_convergence_smac5_mnist}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_secom_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_secom_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_secom_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_secom_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_secom_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset secom.}
    \label{fig:exp_convergence_smac5_secom}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_semeion_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_semeion_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_semeion_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_semeion_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_semeion_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset semeion.}
    \label{fig:exp_convergence_smac5_semeion}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_shuttle_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_shuttle_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_shuttle_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_shuttle_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_shuttle_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset shuttle.}
    \label{fig:exp_convergence_smac5_shuttle}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_waveform_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_waveform_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_waveform_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_waveform_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_waveform_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset waveform.}
    \label{fig:exp_convergence_smac5_waveform}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_winequality_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_winequality_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_winequality_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_winequality_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_winequality_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset winequality.}
    \label{fig:exp_convergence_smac5_winequality}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat[Iter 1]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_yeast_seed0.pdf}
      }%
    \hfill%
    \subfloat[Iter 2]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_yeast_seed1.pdf}
        }%
    \hfill%
    \subfloat[Iter 3]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_yeast_seed2.pdf}
        }%
    \hfill%    
    \subfloat[Iter 4]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_yeast_seed3.pdf}
        }%
    \hfill%
    \subfloat[Iter 5]{%
        \includegraphics[width=0.180\linewidth]{images/img_convergence_smac5_yeast_seed4.pdf}
        }%    
        
        
    \caption{The convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset yeast.}
    \label{fig:exp_convergence_smac5_yeast}
\end{figure*}


\end{landscape}

==> sections/exp_convergence_img_smac5_merged30.tex <==



\begin{figure*}[h] 
   
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_abalone_seed0.pdf}
      }%
    %%\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_abalone_seed1.pdf}
        }%
    %%\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_abalone_seed2.pdf}
        }%
    %%\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_abalone_seed3.pdf}
        }%
    %%\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_abalone_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset abalone.}
    \label{fig:exp_convergence_smac5_abalone}
\end{figure*}











\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_amazon_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_amazon_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_amazon_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_amazon_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_amazon_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset amazon.}
    \label{fig:exp_convergence_smac5_amazon}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_car_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_car_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_car_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_car_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_car_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset car.}
    \label{fig:exp_convergence_smac5_car}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_cifar10small_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_cifar10small_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_cifar10small_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_cifar10small_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_cifar10small_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset cifar10small.}
    \label{fig:exp_convergence_smac5_cifar10small}
\end{figure*}







\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_convex_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_convex_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_convex_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_convex_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_convex_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset convex.}
    \label{fig:exp_convergence_smac5_convex}
\end{figure*}






\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_dorothea_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_dorothea_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_dorothea_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_dorothea_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_dorothea_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset dorothea.}
    \label{fig:exp_convergence_smac5_dorothea}
\end{figure*}


\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gcredit_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gcredit_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gcredit_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gcredit_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gcredit_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset gcredit.}
    \label{fig:exp_convergence_smac5_gcredit}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gisette_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gisette_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gisette_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gisette_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_gisette_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset gisette.}
    \label{fig:exp_convergence_smac5_gisette}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_kddcup_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_kddcup_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_kddcup_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_kddcup_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_kddcup_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset kddcup.}
    \label{fig:exp_convergence_smac5_kddcup}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_krvskp_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_krvskp_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_krvskp_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_krvskp_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_krvskp_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset krvskp.}
    \label{fig:exp_convergence_smac5_krvskp}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_madelon_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_madelon_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_madelon_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_madelon_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_madelon_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset madelon.}
    \label{fig:exp_convergence_smac5_madelon}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_mnist_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_mnist_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_mnist_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_mnist_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_mnist_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset mnist.}
    \label{fig:exp_convergence_smac5_mnist}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_secom_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_secom_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_secom_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_secom_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_secom_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset secom.}
    \label{fig:exp_convergence_smac5_secom}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_semeion_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_semeion_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_semeion_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_semeion_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_semeion_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset semeion.}
    \label{fig:exp_convergence_smac5_semeion}
\end{figure*}





\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_shuttle_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_shuttle_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_shuttle_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_shuttle_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_shuttle_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset shuttle.}
    \label{fig:exp_convergence_smac5_shuttle}
\end{figure*}



\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_waveform_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_waveform_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_waveform_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_waveform_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_waveform_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset waveform.}
    \label{fig:exp_convergence_smac5_waveform}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_winequality_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_winequality_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_winequality_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_winequality_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_winequality_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset winequality.}
    \label{fig:exp_convergence_smac5_winequality}
\end{figure*}




\begin{figure*}[h] 
    \centering
    \subfloat{%
        \includegraphics[width=0.1265\linewidth]{images/smac5_merged/img_convergence_smac5_merged_yeast_seed0.pdf}
      }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_yeast_seed1.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_yeast_seed2.pdf}
        }%
    %\hfill%    
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_yeast_seed3.pdf}
        }%
    %\hfill%
    \subfloat{%
        \includegraphics[width=0.08\linewidth]{images/smac5_merged/img_convergence_smac5_merged_yeast_seed4.pdf}
        }%    
        
        
    \caption{The first 30 minutes of the convergence of the most promising pipelines of SMAC with five initialising configurations using the dataset yeast.}
    \label{fig:exp_convergence_smac5_yeast}
\end{figure*}




==> sections/x.avatar_concept.tex <==

\section{AVATAR Concept}
\label{sec:avatar_concept}



\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{images/avatar_example.pdf}
\vspace{-0.8cm}
\caption{AVATAR Example}
\label{fig:avatar_example}

\end{figure}

Figure \ref{fig:avatar_example} shows an example of how the AVATAR works. The original pipeline is a Weka-based pipeline including three components, EMImputation, IndependentComponents and J48. The input dataset has numeric attributes, missing values in these numeric attributes and nominal class. 

Firstly, the AVATAR maps the Weka-based pipeline to the Petri net based pipeline. The input token for the Petri net based pipeline is token 1. The token is a vector of values 0 and 1. It means that the input data does not have nominal attribute and nominal class (i.e., token value 0, have numeric attribute, missing value attribute and nominal class (i.e., token value 1). The capability (C) and effect (E) of each ML component is retrieved from the AVATAR knowledge base.  

Secondly, executing the Petri net based pipeline will fire all transitions. For example, token 1 has MISSING\_VALUE\_ATTRIBUTE=1. EMImputation has C of  MISSING\_VALUE\_ATTRIBUTE=1. It means that EMImputation can work with missing value attribute. EMImputation has E of MISSING\_VALUE\_ATTRIBUTE=-1. It means that after passing token 1 to EMImputation, the value of MISSING\_VALUE\_ATTRIBUTE is 1 + (-1) = 0 (i.e., the missing values are removed).

If IndependentComponents is put in front of EMImputation, we will have an invalid pipeline. The thing is that IndependentComponents has C of MISSING\_VALUE\_ATTRIBUTE=0, that means it cannot handle missing value attributes.


==> sections/x.exp_results.tex <==
\section{Experiment Results}
\label{sec:exp_results}



Table \ref{tab:exp_awa_2h} presents mean, standard deviation and min of the error rate, and mean, standard deviation (StdDev) and max of the number of evaluated pipelines of 5 iterations with and without the AVATAR using the datasets in Table \ref{tab:exp_datasets}.
We can see that using the AVATAR can accelerate the ML pipeline composition and optimisation. 

\begin{itemize}
    
    \item It's more likely that SMAC can evaluate more pipelines with the AVATAR. The mean of the number of evaluated pipelines is higher than in the cases without the AVATAR in all tested datasets. 
    
    %The AVATAR enables SMAC to evaluate more pipelines. As a result, SMAC integrated the AVATAR is more likely to find better pipelines.
    
    \item It's more likely that SMAC find better pipelines with the AVATAR. Table \ref{tab:exp_awa_2h} shows that mean of the error rate in experiments with the AVATAR is smaller than in the cases without the AVATAR in 15/19 datasets. 

    \item There exists local optimal solutions. Standard deviation of the error rate indicates the degree of the convergence of the runs. The high value of this statistical metric indicates that the runs are more likely to converge to the local optimum. Table \ref{tab:exp_awa_2h} shows there are 4 runs that standard deviation of the error rate in both cases with and without the AVATAR is greater than 5\%. They are the runs using the datasets \textit{amazon}, \textit{cifar10small}, \textit{convex}, and \textit{wquality}. It means that the convergence of the results for these datasets highly depends on the initialisation of SMAC. This initialisation randomly selects first configurations based on seed numbers. 
    
    
\end{itemize}




Table \ref{tab:exp_awa_bestpp} shows the best pipelines of each iteration with and without the AVATAR. This experimental result confirms that the most promising pipelines are often short pipelines (i.e., the pipelines only have one predictor/meta-predictor). There are two cases that the most promising pipelines including data preprocessing components. They are (kddcup09appetency, Iter 1) and (secom, Iter 2).
We try to interpret the semantics of the first pipeline structure, \textit{ClassBalancer $\rightarrow$ RemoveOutliers $\rightarrow$ InterquartileRange $\rightarrow$ AttributeSelection $\rightarrow$ Resample $\rightarrow$ PART}. 
The dataset \textit{kddcup09appetency} is significantly imbalance, therefore, using the ML component \textit{ClassBalancer} can balance the weights of classes. Moreover, this dataset is high dimensional, therefore, using ML components such as \textit{InterquartileRange} and \textit{AttributeSelection} can reduce the number of dimensions. This is a large dataset, therefore, \textit{ReSample} can reduce the size of the dataset to accelerate the training of predictive models. Figure presents the histograms of three selected attributes of this dataset. We see that there are potentially outliers. Therefore, using the component \textit{RemoveOutliers} can remove these outliers and generalise the predictive models better.  









Table \ref{tab:exp_awa_details} shows the error rate and the number of evaluated pipelines of five iterations with and without the AVATAR. We group the experimental results into three main cases.


\begin{itemize}
    \item \textit{The error rate is lower with the AVATAR} (54/95 runs): In this cases, the AVATAR shows its effectiveness to quickly ignore invalid pipelines, therefore, the number of evaluated pipelines are higher than without the AVATAR. As a result, the convergence of SMAC is faster.A n example of these cases is the dataset \texit{cifar10small} with Iter 5. This case clearly shows that the number of evaluated pipelines are higher with the AVATAR, 50 compared to 27. As the result, the error rate is lower with the AVATAR, 64.94 compared to 84.29. 
    
    \item \textit{The same error rate with and without the AVATAR} (37/95 runs):
    \begin{itemize}
        \item \textit{The cases with similar number of evaluated pipelines.} An example of these cases is the dataset \texit{dorothea} with Iter 5. The error rate of both cases is 9.32\% and the number of evaluated pipelines with and without the AVATAR is 21 and 22 and 21 respectively. All of the datasets belong to this type are large and require long training time. Therefore, the number of evaluated pipelines are small. As a result, there is not significant different between the cases with and without the AVATAR.  
        
        %The last pipelines of both cases with and without the AVATAR are terminated because they reach the training time out (1h). 
        
        
        
        \item \textit{The cases with significant different number of evaluated pipelines.} The examples of these cases is the data set \textit{secom} with Iter 1. The error rate of both cases is 6.11\%, and the number of evaluated pipelines with and without the AVATAR are 307 and 108 respectively. We can see the runs are converged quickly with and without the AVATAR because the datasets are quite easy to find well-performing pipelines.
  
    \end{itemize}
    
    \item \textit{The error rate is higher with the AVATAR} (4/95 runs) including (kddcup09appetency, Iter 2), (abalone, Iter 3), (abalone, Iter 4), and (shuttle, Iter 4). The common of these cases is that they have quite a small number of evaluated pipelines and a similar number of evaluated pipelines. The reason is that the training time of these pipelines is significant. Therefore, if the runs with the AVATAR have high complexity pipelines earlier than the runs without the AVATAR, it may trap into these runs until time out.
    
\end{itemize}



Table \ref{tab:exp_awa_details} also shows the incompleted cases (i.e., present by - ) where no result is returned.
The reason is that SMAC has to complete 10 runs for each configuration (i.e., 10-fold cross validation). If only several runs have been completed, the best pipeline will not be returned. In these cases, we do not use these cases to calculate the error rate and relevant metrics.
There are 21 and 39 incompleted cases with and without the AVATAR respectively. The number of incompleted cases is almost double without using the AVATAR. Using the AVATAR can enable SMAC to overcome these situations in 18 over 39 incomplete cases of without the AVATAR.
Overall, we see that the effectiveness of the AVATAR for most of datasets. However, for the datasets and pipelines that require long training time, the integration of the AVATAR does not effectively enable SMAC to find better pipelines. 



\input{tables/exp_awa_2h.tex}

\input{tables/exp_awa_2h_details.tex}

\input{tables/exp_best_pipelines.tex}


Figure \ref{fig:exp_convergence_abalone} to \ref{fig:exp_convergence_yeast} show the convergence of error rate of the runs with different datasets and iterations. We can see that the convergence of the AVATAR is faster or equal without the AVATAR in 93/95 runs.

%, except 2 cases (convex, Iter 4) and (kddcup, Iter 2). 


\input{sections/exp_convergence_img.tex}
\label{sec:exp_results}



Table \ref{tab:exp_awa_2h} presents mean, standard deviation and min of the error rate, and mean, standard deviation (StdDev) and max of the number of evaluated pipelines of 5 iterations with and without the AVATAR using the datasets in Table \ref{tab:exp_datasets}.
We can see that using the AVATAR can accelerate the ML pipeline composition and optimisation. 

\begin{itemize}
    
    \item It's more likely that SMAC can evaluate more pipelines with the AVATAR. The mean of the number of evaluated pipelines is higher than in the cases without the AVATAR in all tested datasets. 
    
    %The AVATAR enables SMAC to evaluate more pipelines. As a result, SMAC integrated the AVATAR is more likely to find better pipelines.
    
    \item It's more likely that SMAC find better pipelines with the AVATAR. Table \ref{tab:exp_awa_2h} shows that mean of the error rate in experiments with the AVATAR is smaller than in the cases without the AVATAR in 15/19 datasets. 

    \item There exists local optimal solutions. Standard deviation of the error rate indicates the degree of the convergence of the runs. The high value of this statistical metric indicates that the runs are more likely to converge to the local optimum. Table \ref{tab:exp_awa_2h} shows there are 4 runs that standard deviation of the error rate in both cases with and without the AVATAR is greater than 5\%. They are the runs using the datasets \textit{amazon}, \textit{cifar10small}, \textit{convex}, and \textit{wquality}. It means that the convergence of the results for these datasets highly depends on the initialisation of SMAC. This initialisation randomly selects first configurations based on seed numbers. 
    
    
\end{itemize}




Table \ref{tab:exp_awa_bestpp} shows the best pipelines of each iteration with and without the AVATAR. This experimental result confirms that the most promising pipelines are often short pipelines (i.e., the pipelines only have one predictor/meta-predictor). There are two cases that the most promising pipelines including data preprocessing components. They are (kddcup09appetency, Iter 1) and (secom, Iter 2).
We try to interpret the semantics of the first pipeline structure, \textit{ClassBalancer $\rightarrow$ RemoveOutliers $\rightarrow$ InterquartileRange $\rightarrow$ AttributeSelection $\rightarrow$ Resample $\rightarrow$ PART}. 
The dataset \textit{kddcup09appetency} is significantly imbalance, therefore, using the ML component \textit{ClassBalancer} can balance the weights of classes. Moreover, this dataset is high dimensional, therefore, using ML components such as \textit{InterquartileRange} and \textit{AttributeSelection} can reduce the number of dimensions. This is a large dataset, therefore, \textit{ReSample} can reduce the size of the dataset to accelerate the training of predictive models. Figure presents the histograms of three selected attributes of this dataset. We see that there are potentially outliers. Therefore, using the component \textit{RemoveOutliers} can remove these outliers and generalise the predictive models better.  









Table \ref{tab:exp_awa_details} shows the error rate and the number of evaluated pipelines of five iterations with and without the AVATAR. We group the experimental results into three main cases.


\begin{itemize}
    \item \textit{The error rate is lower with the AVATAR} (54/95 runs): In this cases, the AVATAR shows its effectiveness to quickly ignore invalid pipelines, therefore, the number of evaluated pipelines are higher than without the AVATAR. As a result, the convergence of SMAC is faster.A n example of these cases is the dataset \texit{cifar10small} with Iter 5. This case clearly shows that the number of evaluated pipelines are higher with the AVATAR, 50 compared to 27. As the result, the error rate is lower with the AVATAR, 64.94 compared to 84.29. 
    
    \item \textit{The same error rate with and without the AVATAR} (37/95 runs):
    \begin{itemize}
        \item \textit{The cases with similar number of evaluated pipelines.} An example of these cases is the dataset \texit{dorothea} with Iter 5. The error rate of both cases is 9.32\% and the number of evaluated pipelines with and without the AVATAR is 21 and 22 and 21 respectively. All of the datasets belong to this type are large and require long training time. Therefore, the number of evaluated pipelines are small. As a result, there is not significant different between the cases with and without the AVATAR.  
        
        %The last pipelines of both cases with and without the AVATAR are terminated because they reach the training time out (1h). 
        
        
        
        \item \textit{The cases with significant different number of evaluated pipelines.} The examples of these cases is the data set \textit{secom} with Iter 1. The error rate of both cases is 6.11\%, and the number of evaluated pipelines with and without the AVATAR are 307 and 108 respectively. We can see the runs are converged quickly with and without the AVATAR because the datasets are quite easy to find well-performing pipelines.
  
    \end{itemize}
    
    \item \textit{The error rate is higher with the AVATAR} (4/95 runs) including (kddcup09appetency, Iter 2), (abalone, Iter 3), (abalone, Iter 4), and (shuttle, Iter 4). The common of these cases is that they have quite a small number of evaluated pipelines and a similar number of evaluated pipelines. The reason is that the training time of these pipelines is significant. Therefore, if the runs with the AVATAR have high complexity pipelines earlier than the runs without the AVATAR, it may trap into these runs until time out.
    
\end{itemize}



Table \ref{tab:exp_awa_details} also shows the incompleted cases (i.e., present by - ) where no result is returned.
The reason is that SMAC has to complete 10 runs for each configuration (i.e., 10-fold cross validation). If only several runs have been completed, the best pipeline will not be returned. In these cases, we do not use these cases to calculate the error rate and relevant metrics.
There are 21 and 39 incompleted cases with and without the AVATAR respectively. The number of incompleted cases is almost double without using the AVATAR. Using the AVATAR can enable SMAC to overcome these situations in 18 over 39 incomplete cases of without the AVATAR.
Overall, we see that the effectiveness of the AVATAR for most of datasets. However, for the datasets and pipelines that require long training time, the integration of the AVATAR does not effectively enable SMAC to find better pipelines. 



\input{tables/exp_awa_2h.tex}

\input{tables/exp_awa_2h_details.tex}

\input{tables/exp_best_pipelines.tex}


Figure \ref{fig:exp_convergence_abalone} to \ref{fig:exp_convergence_yeast} show the convergence of error rate of the runs with different datasets and iterations. We can see that the convergence of the AVATAR is faster or equal without the AVATAR in 93/95 runs.

%, except 2 cases (convex, Iter 4) and (kddcup, Iter 2). 


\input{sections/exp_convergence_img.tex}



==> sections/x.exp_settings.tex <==

\section{Experiment Settings}
\label{sec:exp_settings}



\input{tables/datasets.tex}

Table \ref{tab:exp_datasets} summarises characteristics of datasets\footnote{\url{https://archive.ics.uci.edu}} used for experiments. We use these datasets because they were used in previous studies \cite{sabu18,olmo16,fekl15}. The AutoML tool used for the experiments is AutoWeka4MCPS\footnote{\url{https://github.com/UTS-AAi/autoweka}} integrated the AVATAR.

We run these experiments on AWS EC2 $t3a.medium$ virtual machines which have 2 vCPU and 4GB memory. 
We use five iterations (Iter). Each iteration uses a different seed number. We set the time budget to 2 hours. The memory is set to 1GB. We evaluate the experimental results of the five iterations with (y) and without (n) the AVATAR. We use SMAC as a pipeline composition and optimisation method for all runs. We log the error rate, the pipelines' structure and the number of evaluated pipelines. Besides, we calculate the following criteria:

\begin{itemize}
    \item Mean ($\upmu$), standard deviation ($\upsigma$) and min of the error rate 
    \item Mean ($\upmu$), standard deviation ($\upsigma$) and max of the number of the pipelines
\end{itemize}





==> tables/tab_invalid_pipeline_evidence_autosklearn_old.tex <==


\begin{table}[htb!]

\centering

%\vspace{-0.35cm}

\caption {Negative impacts of invalid pipelines in pipeline composition and optimisation of Auto-sklearn. (1): the number of invalid/ valid pipelines, (2): the total evaluation time of invalid/ valid pipelines (s), (3): the wasted evaluation time (\%).}
\label{tab:neg_impact_invalid_pipeline_autosklearn}
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{Dataset}                 & \textbf{Criteria} & \textbf{Iter 1} & \textbf{Iter 2} & \textbf{Iter 3} & \textbf{Iter 4} & \textbf{Iter 5} \\ \hline
\textbf{abalone}                 & \textbf{}         & crashed         & crashed         & crashed         & crashed         & crashed         \\ \hline
\textbf{car}                     & \textbf{}         & crashed         & crashed         & crashed         & crashed         & crashed         \\ \hline
\multirow{3}{*}{\textbf{convex}} & \textbf{(1)}      & 2/13            & 2/6             & 2/8             & 2/6             & 2/8             \\ \cline{2-7} 
                                 & \textbf{(2)}      & 560.8/2981.8    & 537.7/629.2     & 584.1/1537.5    & 558.1/977.1     & 560.0/1655.9    \\ \cline{2-7} 
                                 & \textbf{(3)}      & 15.76           & 15.07           & 16.39           & 15.66           & 15.72           \\ \hline
\textbf{gcredit}                 & \textbf{}         & crashed         & crashed         & crashed         & crashed         & crashed         \\ \hline
\multirow{3}{*}{\textbf{wineqw}} & \textbf{(1)}      & 0/42            & 0/22            & 0/42            & 0/32            & 0/32            \\ \cline{2-7} 
                                 & \textbf{(2)}      & 0.0/3523.4      & 0.0/909.7       & 0.0/3197.4      & 0.0/3054.0      & 0.0/3163.5      \\ \cline{2-7} 
                                 & \textbf{(3)}      & 0.00            & 0.00            & 0.00            & 0.00            & 0.00            \\ \hline
\end{tabular}
\vspace{-0.35cm}

\end{table}

==> tables/tab_invalid_pipeline_evidence_aw_old.tex <==


\begin{table}[htb!]

\centering


\vspace{-0.35cm}
\caption {Negative impacts of invalid pipelines in pipeline composition and optimisation of AutoWeka4MCPS. (1): the number of invalid/ valid pipelines, (2): the total evaluation time of invalid/ valid pipelines (s), (3): the wasted evaluation time (\%).}
\label{tab:neg_impact_invalid_pipeline_aw}

\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{Dataset}                  & \textbf{Criteria} & \textbf{Iter 1} & \textbf{Iter 2} & \textbf{Iter 3}          & \textbf{Iter 4}          & \textbf{Iter 5}          \\ \hline
\multirow{3}{*}{\textbf{abalone}} & \textbf{(1)}      & 16/26           & 90/79           & 69/88                    & 34/29                    & 53/80                    \\ \cline{2-7} 
                                  & \textbf{(2)}      & 3607.7/1322.5   & 2007.1/1236.4   & 4512.9/2172.3            & 3615.4/277.6             & 23.2/3509.0              \\ \cline{2-7} 
                                  & \textbf{(3)}      & 73.18           & 61.88           & 67.51                    & 92.87                    & 0.66                     \\ \hline
\multirow{3}{*}{\textbf{car}}     & \textbf{(1)}      & 205/152         & 108/70          & 197/313                  & 139/156                  & 85/64                    \\ \cline{2-7} 
                                  & \textbf{(2)}      & 3818.1/291.8    & 3498.5/113.0    & 4523.6/532.6             & 5232.2/251.3             & 4365.1/90.1              \\ \cline{2-7} 
                                  & \textbf{(3)}      & 92.90           & 96.87           & 89.47                    & 95.42                    & 97.98                    \\ \hline
\multirow{3}{*}{\textbf{convex}}  & \textbf{(1)}      & 18/20           & 2/0             & 17/11                    & \multirow{3}{*}{crashed} & \multirow{3}{*}{crashed} \\ \cline{2-5}
                                  & \textbf{(2)}      & 76.3/3588.1     & 3475.2/0.0      & 1324.7/2331.8            &                          &                          \\ \cline{2-5}
                                  & \textbf{(3)}      & 2.08            & 100.00          & 36.23                    &                          &                          \\ \hline
\multirow{3}{*}{\textbf{gcredit}} & \textbf{(1)}      & 112/195         & 229/364         & 208/166                  & 12/54                    & 30/54                    \\ \cline{2-7} 
                                  & \textbf{(2)}      & 2821.0/2260.1   & 3829.8/285.6    & 3933.8/184.0             & 3667.6/34.1              & 3634.8/64.7              \\ \cline{2-7} 
                                  & \textbf{(3)}      & 55.52           & 93.06           & 95.53                    & 99.08                    & 98.25                    \\ \hline
\multirow{3}{*}{\textbf{wineqw}}  & \textbf{(1)}      & 203/213         & 121/139         & \multirow{3}{*}{crashed} & 201/302                  & 36/54                    \\ \cline{2-4} \cline{6-7} 
                                  & \textbf{(2)}      & 4880.6/1052.9   & 4183.4/1078.6   &                          & 2418.5/1132.2            & 1639.2/862.2             \\ \cline{2-4} \cline{6-7} 
                                  & \textbf{(3)}      & 82.26           & 79.50           &                          & 68.11                    & 65.53                    \\ \hline
\end{tabular}
%\vspace{-0.35cm}
\end{table}

==> tables/table_autosklearn_experiments.tex <==

\begin{landscape}

%\begin{table*}[htb!]
\begin{table*}[htb!]

\centering


\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{}                                     & \textbf{seed=0}                                                                                                                      & \textbf{seed=1}                                                                                                                       & \textbf{seed=2}                                                                                                                       & \textbf{seed=3}                                                                                                                      & \textbf{seed=4}                                                                                                                      \\ \hline
\textbf{abalone}                  & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\textbf{amazon}                   & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\textbf{car}                      & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\multirow{3}{*}{\textbf{convex}}  & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding \\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding \\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} \\ \cline{2-7} 
                                  & \textbf{predictor}     & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                     \\ \cline{2-7} 
                                  & \textbf{accuracy}      & 83.36                                                                                                                                & 81.84                                                                                                                                 & \textbf{83.42}                                                                                                                        & 82.73                                                                                                                                & 82.65                                                                                                                                \\ \hline
\multirow{3}{*}{\textbf{dexter}}  & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$LinearSvcPrep\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Normalize\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$LinearSvcPrep\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Normalize\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Normalize\end{tabular}                     \\ \cline{2-7} 
                                  & \textbf{predictor}     & RandomForest                                                                                                                         & SvmSvc                                                                                                                                & RandomForest                                                                                                                          & SvmSvc                                                                                                                               & SvmSvc                                                                                                                               \\ \cline{2-7} 
                                  & \textbf{accuracy}      & 93.33                                                                                                                                & \textbf{96.11}                                                                                                                        & 93.88                                                                                                                                 & 95.56                                                                                                                                & \textbf{96.11}                                                                                                                       \\ \hline
\textbf{dorothea}                 & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\textbf{gcredit}                  & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\multirow{3}{*}{\textbf{gisette}} & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean$\rightarrow$SelectRates\\ $\rightarrow$RobustScaler\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}ImputationMostFrequent\\ $\rightarrow$SelectPercentile\\ $\rightarrow$Standardize\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                                               & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                                              \\ \cline{2-7} 
                                  & \textbf{predictor}     & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                      & RandomForest                                                                                                                          & RandomForest                                                                                                                         & RandomForest                                                                                                                         \\ \cline{2-7} 
                                  & \textbf{accuracy}      & \textbf{97.9}                                                                                                                        & 97.76                                                                                                                                 & 97.57                                                                                                                                 & 97.48                                                                                                                                & 97.1                                                                                                                                 \\ \hline
\multirow{3}{*}{\textbf{shuttle}} & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                    \\ \cline{2-7} 
                                  & \textbf{predictor}     & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                     \\ \cline{2-7} 
                                  & \textbf{accuracy}      & \textbf{99.99}                                                                                                                       & 99.98                                                                                                                                 & \textbf{99.99}                                                                                                                        & \textbf{99.99}                                                                                                                       & \textbf{99.99}                                                                                                                       \\ \hline
\multirow{3}{*}{\textbf{wineqw}}  & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                 \\ \cline{2-7} 
                                  & \textbf{predictor}     & Adaboost                                                                                                                             & Adaboost                                                                                                                              & Adaboost                                                                                                                              & Adaboost                                                                                                                             & Adaboost                                                                                                                             \\ \cline{2-7} 
                                  & \textbf{accuracy}      & \textbf{65.83}                                                                                                                       & \textbf{65.83}                                                                                                                        & \textbf{65.83}                                                                                                                        & \textbf{65.83}                                                                                                                       & \textbf{65.83}                                                                                                                       \\ \hline
\end{tabular}

\caption {Pipeline structure and accuracy in percentage generated by Auto-sklearn using different datasets and seed numbers}
\label{tab:autosklearn_exp}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_autoweka_experiments.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
                                   &                        & \textbf{seed=0}                                                         & \textbf{seed=1}                                                           & \textbf{seed=2}                                                                                                                    & \textbf{seed=3}                                                      & \textbf{seed=4}                                                         \\ \hline
\multirow{3}{*}{\textbf{abalone}}  & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ Ranker\end{tabular} & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular} \\ \cline{2-7} 
                                   & \textbf{predictor}     & trees.LMT                                                               & bayes.BayesNet                                                            & \begin{tabular}[c]{@{}l@{}}functions.\\ MultilayerPerceptron\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}functions.\\ SimpleLogistic\end{tabular}  & trees.LMT                                                               \\ \cline{2-7} 
                                   & \textbf{accuracy}      & 25.62                                                                   & 26.02                                                                     & \textbf{26.18}                                                                                                                     & 25.62                                                                & 25.94                                                                   \\ \hline
\multirow{3}{*}{\textbf{amazon}}   & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular} \\ \cline{2-7} 
                                   & \textbf{predictor}     & bayes.NaiveBayes                                                        & -                                                                         & rules.PART                                                                                                                         & -                                                                    & trees.J48                                                               \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{62.22}                                                          & -                                                                         & 34.67                                                                                                                              & -                                                                    & 21.78                                                                   \\ \hline
\multirow{3}{*}{\textbf{car}}      & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular} & -                                                                         & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular}                                                            & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & functions.SMO                                                           & trees.J48                                                                 & functions.SMO                                                                                                                      & trees.LMT                                                            & functions.SMO                                                           \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{100.00}                                                         & 96.14                                                                     & \textbf{100.00}                                                                                                                    & 97.68                                                                & 97.68                                                                   \\ \hline
\multirow{3}{*}{\textbf{convex}}   & \textbf{preprocessors} & -                                                                       & -                                                                         & \begin{tabular}[c]{@{}l@{}}attribute.Center \rightarrow\\ attribute.PrincipalComponents\\ \rightarrow instance.PeriodicSampling\end{tabular} & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & trees.J48                                                               & -                                                                         & \begin{tabular}[c]{@{}l@{}}meta.\\ ClassificationViaRegression\end{tabular}                                                        & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{62.44}                                                          & {\ul -}                                                                   & 50.29                                                                                                                              & \textbf{-}                                                           & -                                                                       \\ \hline
\multirow{3}{*}{\textbf{dexter}}   & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & \begin{tabular}[c]{@{}l@{}}bayes.\\ NaiveBayesMultinomial\end{tabular}  & -                                                                         & -                                                                                                                                  & rules.Jrip                                                           & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{89.44}                                                          & {\ul -}                                                                   & -                                                                                                                                  & 86.67                                                                & -                                                                       \\ \hline
\multirow{3}{*}{\textbf{dorothea}} & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & rules.OneR                                                              & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{94.49}                                                          & -                                                                         & {\ul -}                                                                                                                            & -                                                                    & -                                                                       \\ \hline
\multirow{3}{*}{\textbf{gcredit}}  & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ Ranker\end{tabular}    \\ \cline{2-7} 
                                   & \textbf{predictor}     & bayes.NaiveBayes                                                        & \begin{tabular}[c]{@{}l@{}}functions.\\ MultilayerPerceptron\end{tabular} & functions.SMO                                                                                                                      & bayes.NaiveBayes                                                     & \begin{tabular}[c]{@{}l@{}}functions.\\ Logistic\end{tabular}           \\ \cline{2-7} 
                                   & \textbf{accuracy}      & 69.33                                                                   & 50.05                                                                     & 70.33                                                                                                                              & 69.33                                                                & \textbf{73.67}                                                          \\ \hline
\multirow{3}{*}{\textbf{gisette}}  & \textbf{preprocessors} & attributeSelection.Ranker                                               & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & trees.REPTree                                                           & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{93.52}                                                          & -                                                                         & -                                                                                                                                  & -                                                                    & {\ul -}                                                                 \\ \hline
\end{tabular}


\caption {Pipeline structure and accuracy(\%) generated by AutoWeka4MCPS using different datasets and seed numbers}
\label{tab:autoweka_exp}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_capabilities.tex <==
\begin{table}[]
\begin{tabular}{l|l}
\hline
\textbf{Algorithm capability/ Dataset meta-feature} & \textbf{Description}                         \\ \hline \hline
BINARY\_ATTRIBUTES                                       & can handle binary attributes                 \\ \hline
BINARY\_CLASS                                            & can handle binary classes                    \\ \hline
DATE\_ATTRIBUTES                                         & can handle date attributes                   \\ \hline
DATE\_CLASS                                              & can handle date classes                      \\ \hline
EMPTY\_NOMINAL\_ATTRIBUTES                               & can handle empty nominal attributes          \\ \hline
EMPTY\_NOMINAL\_CLASS                                    & can handle empty nominal classes             \\ \hline
MISSING\_CLASS\_VALUES                                   & can handle missing values in class attribute \\ \hline
MISSING\_VALUES                                          & can handle missing values in attributes      \\ \hline
NOMINAL\_ATTRIBUTES                                      & can handle nominal attributes                \\ \hline
NOMINAL\_CLASS                                           & can handle nominal classes                   \\ \hline
NUMERIC\_ATTRIBUTES                                      & can handle numeric attributes                \\ \hline
NUMERIC\_CLASS                                           & can handle numeric classes                   \\ \hline
STRING\_CLASS                                            & can handle string classes                    \\ \hline
UNARY\_ATTRIBUTES                                        & can handle unary attributes                  \\ \hline
UNARY\_CLASS                                             & can handle unary classes                     \\ \hline
OUTLIER                                                  & can handle outlier                           \\ \hline
\end{tabular}

\caption {List of algorithms' capabilities or dataset meta-features}
\label{tab:capabilities}
\vspace{-0.5cm}
\end{table}

==> tables/table_component_valid_check.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Input token:\\ meta-feature X\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Algorithm\\ capability X\end{tabular}} & \textbf{Validity} \\ \hline
1                                                                              & 1                                                                         & Valid             \\ \hline
0                                                                              & 0                                                                         & Valid             \\ \hline
1                                                                              & 0                                                                         & Invalid           \\ \hline
0                                                                              & 1                                                                         & Valid             \\ \hline
\end{tabular}
\caption {Rules for checking validity of one activity/component in a pipeline}
\label{tab:component_valid}
\vspace{-0.5cm}
\end{table}

==> tables/table_dataset.tex <==
\begin{table}[htb!]
\centering



\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{\#}} & \multicolumn{6}{l|}{\textbf{attributes}}                                                                  & \multicolumn{4}{l|}{\textbf{class}}                                  \\ \cline{2-11} 
                             & \textbf{n\_num} & \textbf{n\_bin} & \textbf{n\_nom} & \textbf{n\_ept} & \textbf{\%miss} & \textbf{n\_rdd} & \textbf{type} & \textbf{distinct} & \textbf{\%miss} & \textbf{distr} \\ \hline
1                            & 1               & 1               & 1               & 1               & 5\%             & 1               & nominal       & 3                 & 5\%             & 9:1            \\ \hline
2                            & 2               & 0               & 0               & 0               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
3                            & 0               & 2               & 0               & 0               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
4                            & 0               & 0               & 2               & 0               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
5                            & 1               & 0               & 0               & 1               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
6                            & 2               & 0               & 0               & 0               & 5\%             & 0               & nominal       & 3                 & 0               & bal            \\ \hline
7                            & 2               & 0               & 0               & 0               & 0               & 1               & nominal       & 3                 & 0               & bal            \\ \hline
8                            & 2               & 0               & 0               & 0               & 0               & 0               & nominal       & 3                 & 5\%             & bal            \\ \hline
9                            & 2               & 0               & 0               & 0               & 0               & 0               & nominal       & 3                 & 0               & 9:1            \\ \hline
10                           & 2               & 0               & 0               & 0               & 0               & 0               & binary        & n/a               & 0               & bal            \\ \hline
11                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & n/a               & 0               & n/a            \\ \hline
12                           & 1               & 1               & 1               & 1               & 5\%             & 1               & numeric       & 3                 & 5\%             & 9:1            \\ \hline
13                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
14                           & 0               & 2               & 0               & 0               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
15                           & 0               & 0               & 2               & 0               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
16                           & 1               & 0               & 0               & 1               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
17                           & 2               & 0               & 0               & 0               & 5\%             & 0               & numeric       & 3                 & 0               & bal            \\ \hline
18                           & 2               & 0               & 0               & 0               & 0               & 1               & numeric       & 3                 & 0               & bal            \\ \hline
19                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & 3                 & 5\%             & bal            \\ \hline
20                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & 3                 & 0               & 9:1            \\ \hline
\end{tabular}



\caption {Synthetic datasets for generating meta-knowledge. Number of instances (instances), number of numeric attributes (n\_num), number of binary attributes (n\_bin), number of nominal attributes (n\_nom), number of empty attributes (n\_ept), percentage of missing values of attributes (attributes - \%miss), number of redundant attributes (n\_rdd), type of class (type), number of distinct values for nominal class (distinct), percentage of missing values of class (class - \%miss), distribution of class (distr), balance (bal), imbalanced with ratio x/y (x:y), not available (n/a).}
\label{tab:dataset}
\vspace{-0.5cm}
\end{table}

==> tables/table_dataset_description.tex <==
\begin{table}[htb!]

\vspace{-0.35cm}
\caption {Summary of datasets' characteristics: the number of numeric attributes, nominal attributes, distinct classes, instances in training and testing sets.}
\label{tab:exp_datasets}


\centering
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Dataset} & \textbf{Numeric} & \textbf{Nominal} & \textbf{No of distinct classes} & \textbf{Training} & \textbf{Testing} \\ \hline
abalone          & 7                & 1                & 26                              & 2,924          & 1,253         \\ \hline
car              & 0                & 6                & 4                               & 1,210          & 518           \\ \hline
convex           & 784              & 0                & 2                               & 8,000          & 50,000        \\ \hline
gcredit          & 7                & 13               & 2                               & 700            & 300           \\ \hline
wineqw           & 11               & 0                & 7                               & 3,429          & 1,469         \\ \hline
\end{tabular}

\vspace{-0.35cm}


\end{table}

==> tables/table_exp_avatar_evaluation_time.tex <==
\begin{table}[htb!]
\caption {Comparison of the number of total evaluated, valid and invalid pipelines generated during the random search (RS), and the average evaluation time in ms of all, valid and invalid pipelines using T-method, AVATAR and AutoWeka4MCPS}
\label{tab:exp_avatar_evaluation_time}
\vspace{-0.2cm}


\resizebox{\textwidth}{!}{%
\centering

\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Total\\ evaluated\\ pipelines\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Valid\\ pipelines\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Invalid\\ pipelines\end{tabular}}} & \multicolumn{3}{l|}{\textbf{Average evaluation time (ms)}}                                                                                                                                                   \\ \cline{6-8} 
                                  &                                  &                                                                                                 &                                                                                     &                                                                                       & \textbf{\begin{tabular}[c]{@{}l@{}}All\\ pipelines\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Valid\\ pipelines\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Invalid\\ pipelines\end{tabular}} \\ \hline
\multirow{2}{*}{abalone}          & T-method                         & 72                                                                                              & 14                                                                                  & 58                                                                                    & 73,441                                                           & 176,912                                                            & 48,465                                                               \\ \cline{2-8} 
                                  & AVATAR                           & 131                                                                                             & 20                                                                                  & 111                                                                                   & 32,482                                                           & 210,908                                                            & 333                                                                  \\ \hline
\multirow{2}{*}{car}              & T-method                         & 733                                                                                             & 208                                                                                 & 525                                                                                   & 4,933                                                            & 13,362                                                             & 1,594                                                                \\ \cline{2-8} 
                                  & AVATAR                           & 891                                                                                             & 230                                                                                 & 661                                                                                   & 4,032                                                            & 14,967                                                             & 227                                                                  \\ \hline
\multirow{2}{*}{convex}           & T-method                         & 67                                                                                              & 10                                                                                  & 57                                                                                    & 53,936                                                           & 75,666                                                             & 50,124                                                               \\ \cline{2-8} 
                                  & AVATAR                           & 47                                                                                              & 9                                                                                   & 38                                                                                    & 114,791                                                          & 543,284                                                            & 13,306                                                               \\ \hline
\multirow{2}{*}{gcredit}          & T-method                         & 363                                                                                             & 102                                                                                 & 261                                                                                   & 13,451                                                           & 39,191                                                             & 3,392                                                                \\ \cline{2-8} 
                                  & AVATAR                           & 1,018                                                                                           & 244                                                                                 & 774                                                                                   & 4,663                                                            & 17,083                                                             & 748                                                                  \\ \hline
\multirow{2}{*}{wineqw}           & T-method                         & 200                                                                                             & 60                                                                                  & 140                                                                                   & 18,967                                                           & 34,988                                                             & 12,101                                                               \\ \cline{2-8} 
                                  & AVATAR                           & 549                                                                                             & 63                                                                                  & 486                                                                                   & 13,787                                                           & 101,620                                                            & 2,401                                                                \\ \hline
\end{tabular}

}


\end{table}




==> tables/table_exp_result_analyse.tex <==
\begin{table}[htb!]
\centering

\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Configs}                                                                         & \textbf{Tools}    & \textbf{n\_best} & \textbf{n\_worst} & \textbf{n\_fail} & \textbf{min\_diff} & \textbf{max\_diff} & \textbf{avg\_diff} \\ \hline
\multirow{7}{*}{\textbf{1 hour}}                                                         & \textbf{AW}       & 2                & 0                 & 1                & \textbf{0}         & \textbf{-13.59}    & -2.63818           \\ \cline{2-8} 
                                                                                         & \textbf{AW2}      & 1                & 1                 & 1                & \textbf{0}         & -41.11             & -5.97091           \\ \cline{2-8} 
                                                                                         & \textbf{AW4MP}    & 0                & 0                 & 1                & -0.02              & -19.11             & -4.70273           \\ \cline{2-8} 
                                                                                         & \textbf{A-SKL}    & 2                & 0                 & 4                & \textbf{0}         & -39.25             & -5.675             \\ \cline{2-8} 
                                                                                         & \textbf{H2O}      & 2                & 0                 & 3                & \textbf{0}         & -41.95             & -9.32222           \\ \cline{2-8} 
                                                                                         & \textbf{TPOT}     & 1                & 0                 & 2                & \textbf{0}         & -40.38             & -6.782             \\ \cline{2-8} 
                                                                                         & \textbf{MathTC}   & 2                & 0                 & 0                & \textbf{0}         & -38.8              & -5.53083           \\ \hline
\multirow{7}{*}{\textbf{24 hours}}                                                       & \textbf{AW}       & 2                & 0                 & 0                & \textbf{0}         & -15.32             & -3.2175            \\ \cline{2-8} 
                                                                                         & \textbf{AW2}      & 1                & 0                 & 1                & \textbf{0}         & -37.33             & -6.78727           \\ \cline{2-8} 
                                                                                         & \textbf{AW4MP}    & 2                & 0                 & 0                & \textbf{0}         & -17.59             & \textbf{-2.38083}  \\ \cline{2-8} 
                                                                                         & \textbf{A-SKL}    & 2                & 0                 & 4                & \textbf{0}         & -38.58             & -5.1025            \\ \cline{2-8} 
                                                                                         & \textbf{H2O}      & 0                & 0                 & 5                & -0.15              & -44.65             & -12.38             \\ \cline{2-8} 
                                                                                         & \textbf{TPOT}     & 0                & 0                 & 2                & -0.21              & -38.13             & -6.685             \\ \cline{2-8} 
                                                                                         & \textbf{MathTC}   & 1                & 0                 & 0                & \textbf{0}         & -38.58             & -6.176             \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}No\\ time\\ constraint\end{tabular}}} & \textbf{MLBox}    & 1                & 0                 & 2                & \textbf{0}         & -40.38             & -7.377             \\ \cline{2-8} 
                                                                                         & \textbf{AutoML}   & 1                & 0                 & 0                & \textbf{0}         & -31.16             & -6.88083           \\ \cline{2-8} 
                                                                                         & \textbf{RM}       & 0                & 1                 & 0                & -0.07              & -32                & -7.24              \\ \cline{2-8} 
                                                                                         & \textbf{ATM}      & 1                & 1                 & 1                & \textbf{0}         & -41.05             & -11.0309           \\ \cline{2-8} 
                                                                                         & \textbf{AWS ML}   & 1                & 1                 & 2                & \textbf{0}         & -38.13             & -12.598            \\ \hline
\multirow{4}{*}{\textbf{Baselines}}                                                      & \textbf{NBayes}   & 0                & 5                 & 0                & -7                 & {\underline{-59.7}}        & {\underline{-25.56}}       \\ \cline{2-8} 
                                                                                         & \textbf{LogReg}   & 0                & 3                 & 0                & {\underline{-0.43}}        & -40.15             & -15.3942           \\ \cline{2-8} 
                                                                                         & \textbf{RdForest} & 1                & 0                 & 0                & \textbf{0}         & -39.7              & -7.74833           \\ \cline{2-8} 
                                                                                         & \textbf{XGBoost}  & 1                & 0                 & 0                & \textbf{0}         & -39.03             & -8.34833           \\ \hline
\end{tabular}



\caption {Experimental results of the AutoML tools: number of the best predictive models (n\_best), number of the worst predictive models (n\_worst), number of failed cases (n\_fail), minimum difference from the best predictive model (min\_diff), maximum difference from the best predictive model (max\_diff), and average difference from the best predictive model (avg\_diff)  }



\label{tab:exp_results_analyse}
\vspace{-0.5cm}
\end{table}

==> tables/table_generate_pipeline_method_compare.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering





\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Method}}                                 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Pipeline\\ structure\end{tabular}}} & \multicolumn{3}{l|}{\textbf{Max components by type}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Max\\ length\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Knowledge for\\ construction\end{tabular}}} & \multicolumn{3}{l|}{\textbf{Libraries/algorithms}}       & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Hyperparameter\\ Optimization\end{tabular}}}     \\ \cline{3-5} \cline{8-10}
                                                                 &                                                                                        & \textbf{Prep}    & \textbf{Pred}   & \textbf{Ense}   &                                                                                &                                                                                                & \textbf{Prep}            & \textbf{Pred} & \textbf{ense} &                                                                                                     \\ \hline
\begin{tabular}[c]{@{}l@{}}Auto-weka \\ v0.5/v2.0\end{tabular}   & SW                                                                                     & 1                & 1               & 1               & 3                                                                              & fixed                                                                                          & 3                        & 36            & 0             & SMAC                                                                                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Auto-weka\\ for MCPS\end{tabular}     & SW                                                                                     & 5                & 1               & 1               & 7                                                                              & fixed                                                                                          & 17                       & 34            & 0             & SMAC                                                                                                \\ \hline
Auto-sklearn                                                     & SW                                                                                     & 4                & 1               & 0               & 5                                                                              & fixed                                                                                          & 18                       & 15            & 1             & SMAC                                                                                                \\ \hline
Bolme et al.                                                     & SW                                                                                     & 1                & 1               & 0               & 2                                                                              & fixed                                                                                          & 1                        & 1             & NA            & GP                                                                                                  \\ \hline
RECIPE                                                           & \begin{tabular}[c]{@{}l@{}}derivation\\ tree\end{tabular}                              & ul               & ul              & 1               & ul                                                                             & CFG                                                                                            & 33                       & 23            & 4             & Random search                                                                                       \\ \hline
GRADIENT                                                         & tree                                                                                   & 0                & ul              & ul              & ul                                                                             & CFG                                                                                            & NA                       & NA            & NA            & GP                                                                                                  \\ \hline
TPOT                                                             & tree                                                                                   & ul               & 1               & 1               & ul                                                                             & NA                                                                                             & 19                       & 11            & 0             & \begin{tabular}[c]{@{}l@{}}Pareto\\ optimization\end{tabular}                                       \\ \hline
Layered-TPOT                                                     & tree                                                                                   & ul               & 1               & 1               & ul                                                                             & NA                                                                                             & NA                       & NA            & NA            & \begin{tabular}[c]{@{}l@{}}Pareto\\ optimization\end{tabular}                                       \\ \hline
Kordik et al.                                                    & tree                                                                                   & 0                & ul              & ul              & ul                                                                             & CFG                                                                                            & 0                        & 5             & 7             & GP                                                                                                  \\ \hline
ML-Plan                                                          & SW                                                                                     & ul               & 1               & 1               & ul                                                                             & HTN search space                                                                               & 25                       & 42            & 0             & Random search                                                                                       \\ \hline
ML-Plan-UL                                                       & SW                                                                                     & ul               & ul              & 1               & ul                                                                             & HTN search space                                                                               & 25                       & 42            & 3             & Random search                                                                                       \\ \hline
MLS-Plan                                                         & SW                                                                                     & ul               & 1               & 1               & ul                                                                             & HTN search space                                                                               & \multicolumn{3}{l|}{NA}                                  & Random search                                                                                       \\ \hline
P4ML                                                             & SW                                                                                     & yes              & yes             & yes             & NA                                                                             & \begin{tabular}[c]{@{}l@{}}A catalog \\ of primitives\end{tabular}                             & \multicolumn{1}{c|}{127} &               &               & NA                                                                                                  \\ \hline
AutoComplete                                                     & tree                                                                                   & NA               & ul              & 1               & ul                                                                             & fixed                                                                                          & NA                       & 14            & 1             & \begin{tabular}[c]{@{}l@{}}Random search \\ or grid search\end{tabular}                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Automatic\\ Frankenstein\end{tabular} & tree                                                                                   & 0                & ul              & 1               & ul                                                                             & \begin{tabular}[c]{@{}l@{}}Meta-learning from \\ historical runs\end{tabular}                  & NA                       & NA            & NA            & \begin{tabular}[c]{@{}l@{}}Meta-learning\\ + model selection \\ + weighted \\ ensemble\end{tabular} \\ \hline
AutoBagging                                                      & tree                                                                                   & 0                & NA              & NA              & NA                                                                             & fixed                                                                                          & NA                       & NA            & NA            & \begin{tabular}[c]{@{}l@{}}Meta-learning \\ + average rank \\ of models\end{tabular}                \\ \hline
\end{tabular}





\caption {Comparison of the pipeline composition and optimisation methods in term of pipeline structure, max number of components by type in a pipeline (preprocessor, predictor, and ensemble), max length of a pipeline, knowledge for pipeline construction, libraries/algorithms used for implementation (preprosessor, predictor, and ensemble), hyperparameter optimisation method. SW: sequential workflow, ul: unlimited length, HTN: hierarchical task network, CFG: context free grammars, NA: not available, GP: genetic programming, fixed: fixed template.}
\label{tab:method_compare}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_io_convert.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Input token: \\ meta-feature X\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Algorithm\\ capability X\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Output token:\\ meta-feature X\end{tabular}} \\ \hline
1                                                                               & 1                                                                         & 0                                                                               \\ \hline
0                                                                               & 0                                                                         & 0                                                                               \\ \hline
1                                                                               & 0                                                                         & 1                                                                               \\ \hline
0                                                                               & 1                                                                         & 0                                                                               \\ \hline
\end{tabular}
\caption {Rules to calculate output token from input token and algorithm capabilities}
\label{tab:io_convert}
\vspace{-0.5cm}
\end{table}

==> tables/table_methods_compare.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering
%\small


\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{\#}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{l|}{\textbf{Predict model}} & \multicolumn{4}{l|}{\textbf{Search space's characteristics}}         & \multicolumn{3}{l|}{\textbf{Search space tructure}} & \multicolumn{4}{l|}{\textbf{Approach to find best model}}             \\ \cline{3-15} 
                             &                                  & \textbf{Cls}          & \textbf{Regrs}         & \textbf{Prep} & \textbf{Clsfier} & \textbf{M-clsfier} & \textbf{Hyp} & \textbf{Func}   & \textbf{Tree}   & \textbf{Graph}  & \textbf{BayesOpt} & \textbf{HPlan} & \textbf{Rand} & \textbf{M-learn} \\ \hline
1                            & ROAR                             & -                     & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & -               & -               & -                 & -              & $\checkmark$  & -                \\ \hline
2                            & SMAC                             & $\checkmark$          & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
3                            & TPE                              & -                     & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
4                            & CASH                             & $\checkmark$          & $\checkmark$           & -             & $\checkmark$     & -                  & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
5                            & MCPS                             & $\checkmark$          & $\checkmark$           & $\checkmark$  & $\checkmark$     & $\checkmark$       & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
6                            & Spearmint                        & -                     & $\checkmark$           & -             & -                & -                  & $\checkmark$ & $\checkmark$    & -               & -               & $\checkmark$      & -              & -             & -                \\ \hline
7                            & HyperBand                        & $\checkmark$          & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & -               & -               & -                 & -              & $\checkmark$  & -                \\ \hline
8                            & ML-Plan                          & $\checkmark$          & $\checkmark$           & $\checkmark$  & $\checkmark$     & $\checkmark$       & $\checkmark$ & -               & -               & $\checkmark$    & -                 & $\checkmark$   & -             & -                \\ \hline
9                            & AR*                              & $\checkmark$          & $\checkmark$           & -             & $\checkmark$     & -                  & $\checkmark$ & -               & -               & -               & -                 & -              & -             & $\checkmark$     \\ \hline
10                           & Auto-sklearn                     & $\checkmark$          & $\checkmark$           & $\checkmark$  & $\checkmark$     & $\checkmark$       & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & $\checkmark$     \\ \hline
\end{tabular}


\caption {Compare composition and optimisation methods for machine learning pipelines in term of predictive model type (classification or regression), characteristics of search space (preprocessing, classifier, meta-classifier and hyper-parameters), structure of search space (based on function, tree, and graph) and approaches to find best predictive models (based on Bayesian optimisation, hierarchical planning, random and meta-learning) }
\label{tab:method_compare}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_performance.tex <==
\begin{landscape}
\begin{table*}[htb!]
\centering

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{dataset}}                                                                 & \textbf{abalone} & \textbf{amazon} & \textbf{car}    & \textbf{\begin{tabular}[c]{@{}l@{}}german\\ credit\end{tabular}} & \textbf{gisette} & \textbf{krvskp} & \textbf{madelon} & \textbf{semeion} & \textbf{shuttle} & \textbf{\begin{tabular}[c]{@{}l@{}}wave\\ form\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}wine\\ qw\end{tabular}} & \textbf{yeast} \\ \hline
\multirow{7}{*}{\textbf{1h}}                                                        & \textbf{AW}      & 22.91            & -               & 99.81           & 72.33                                                            & 97.33            & 99.48           & 73.72            & 93.50            & \textbf{99.99}   & 85.60                                                        & \textbf{67.19}                                             & 62.02          \\ \cline{2-14} 
                                                                                    & \textbf{AW2}     & 25.94            & \underline{40.22}     & \textbf{100.00} & 71.00                                                            & 95.29            & 99.58           & -                & 90.36            & 99.86            & 85.93                                                        & 63.51                                                      & 59.55          \\ \cline{2-14} 
                                                                                    & \textbf{AW4MP}    & 22.83            & 62.22           & 98.46           & 72.33                                                            & -                & 99.37           & 79.10            & 91.82            & 99.97            & 85.80                                                        & 65.21                                                      & 57.53          \\ \cline{2-14} 
                                                                                    & \textbf{A-SKL}   & -                & -               & 99.03           & \textbf{75.00}                                                   & 97.38            & 99.48           & 83.08            & 94.76            & -                & \textbf{86.33}                                               & -                                                          & 23.15          \\ \cline{2-14} 
                                                                                    & \textbf{H20}     & -                & 48.00           & 98.65           & 71.67                                                            & 97.71            & \textbf{99.79}  & -                & -                & \textbf{99.99}   & 85.33                                                        & 64.40                                                      & 20.45          \\ \cline{2-14} 
                                                                                    & \textbf{TPOT}    & 25.94            & -               & 98.65           & 73.00                                                            & -                & 99.37           & 83.97            & 92.66            & \textbf{99.99}   & 85.53                                                        & 56.09                                                      & 22.02          \\ \cline{2-14} 
                                                                                    & \textbf{MathTC}  & 25.38            & \textbf{81.33}  & 98.46           & 72.00                                                            & 97.67            & 99.16           & 82.95            & 89.52            & \textbf{99.99}   & 83.27                                                        & 64.53                                                      & 23.60          \\ \hline
\multirow{7}{*}{\textbf{24h}}                                                       & \textbf{AW}      & 26.49            & 66.01           & 99.60           & 71.76                                                            & 97.76            & 99.69           & 78.44            & \textbf{94.92}   & \textbf{99.99}   & 85.58                                                        & 66.05                                                      & 59.33          \\ \cline{2-14} 
                                                                                    & \textbf{AW2}     & 25.14            & 44.00           & \textbf{100.00}    & 70.67                                                            &                  & 99.48           & 79.23            & 87.42            & 99.86            & 86.13                                                        & 63.38                                                      & 56.4           \\ \cline{2-14} 
                                                                                    & \textbf{AW4MP}    & 26.59            & 63.74           & 99.9            & 74.58                                                            & 97.66            & 99.77           & 83.20            & 94.90            & \textbf{99.99}   & 85.83                                                        & 67.10                                                      & \textbf{62.40} \\ \cline{2-14} 
                                                                                    & \textbf{A-SKL}   & -                & -               & 99.61           & 74.67                                                            & \textbf{97.86}   & 99.58           & \textbf{87.31}   & 94.34            & -                & 85.60                                                        & -                                                          & 23.82          \\ \cline{2-14} 
                                                                                    & \textbf{H20}     & -                & 62.67           & -               & 72.67                                                            & 97.71            & -               & -                & 93.50            & -                & 85.33                                                        & 48.74                                                      & 17.75          \\ \cline{2-14} 
                                                                                    & \textbf{TPOT}    & 25.94            & -               & 97.88           & 73.00                                                            & 97.14            & 99.58           & 83.97            & 92.66            & -                & 85.53                                                        & 56.09                                                      & 24.27          \\ \cline{2-14} 
                                                                                    & \textbf{MathTC}  & 25.06            & -               & 99.42           & 71.67                                                            & -                & 99.58           & 82.95            & 90.99            & \textbf{99.99}   & 85.27                                                        & 64.53                                                      & 23.82          \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}no\\ time\\ limit\end{tabular}}} & \textbf{MLBox}   & 24.50            & -               & 94.40           & 73.33                                                            & -                & 99.06           & 82.82            & 90.57            & \textbf{99.99}   & 83.93                                                        & 60.65                                                      & 22.02          \\ \cline{2-14} 
                                                                                    & \textbf{AutoML}  & 25.78            & 63.56           & 95.75           & 74.67                                                            & 97.33            & 99.06           & 71.67            & 91.19            & \textbf{99.99}   & 85.73                                                        & 65.69                                                      & 31.24          \\ \cline{2-14} 
                                                                                    & \textbf{RapidM}  & -                & 49.33           & 98.84           & \underline{66.33}                                                      & 96.95            & 97.39           & 81.15            & 89.10            & 99.92            & 85.40                                                        & 62.90                                                      & 45.17          \\ \cline{2-14} 
                                                                                    & \textbf{ATM}     & -                & 56.89           & 97.88           & 72.67                                                            & 96.52            & 97.29           & 67.56            & 83.23            & \textbf{99.99}   & \underline{76.20}                                                  & 61.20                                                      & 21.35          \\ \cline{2-14} 
                                                                                    & \textbf{AWS ML}  & \textbf{32.11}   & -               & 86.87           & 70.00                                                            & -                & 90.29           & \underline{52.31}      & 90.36            & 99.91            & 82.77                                                        & 50.17                                                      & 24.27          \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}base\\ line\end{tabular}}}       & \textbf{NBayes}      & 11.33            & 48.22           & 66.02           & 68.00                                                            & \underline{74.10}      & \underline{59.81}     & 63.59            & \underline{77.15}      & \underline{82.66}      & 78.80                                                        & 45.13                                                      & \underline{2.70}     \\ \cline{2-14} 
                                                                                    & \textbf{LogReg}      & \underline{10.00}      & 74.22           & \underline{63.90}     & 67.00                                                            & 97.43            & 96.66           & 55.38            & 89.73            & 95.19            & 85.53                                                        & \underline{42.21}                                                & 22.25          \\ \cline{2-14} 
                                                                                    & \textbf{RdForest}      & 23.46            & 64.89           & 98.84           & 70.33                                                            & 97.10            & 98.85           & 72.82            & 92.03            & \textbf{99.99}   & 83.73                                                        & 66.51                                                      & 22.70          \\ \cline{2-14} 
                                                                                    & \textbf{XGBoost} & 25.86            & 70.67           & 94.21           & 70.67                                                            & 97.24            & 97.39           & 73.72            & 90.36            & \textbf{99.99}   & 83.80                                                        & 56.77                                                      & 23.37          \\ \hline
\end{tabular}


\caption {Experimental results of AutoML tools: AutoWeka v0.5 - SMAC (AW), AutoWeka v2.6.1 - SMAC (AW2), AutoWeka for MCPS - SMAC (AW4MP), Auto-sklearn (A-SKL), H20, TPOT, Mathematica (MathTC), MLBox, AutoML, RapidMiner (RapidM), ATM, AWS Machine Learning (AWS ML), Naive Bayes (NBayes), Logistic Regression (LogReg), Random Forest (RdForest) and XGBoost}
\label{tab:exp_results}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_pipeline_modeling.tex <==
\begin{table}[htb!]





\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{Method}                                                                       & \textbf{\begin{tabular}[c]{@{}l@{}}Function\\ composition\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Directed\\ acyclic\\ graphs\end{tabular}} & \textbf{Petri nets} & \textbf{OWL-S} & \textbf{BPMN} & \textbf{BPEL} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Easily\\ understandable\\ by human\end{tabular}}   & no                                                                      & yes                                                                          & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Easily\\ understandable\\ by machine\end{tabular}} & yes                                                                     & no                                                                           & no                  & no             & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Support different\\ component types\end{tabular}}  & abstract                                                                & abstract                                                                     & abstract            & no             & yes           & no            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Modeling \\ data flow\end{tabular}}                & yes                                                                     & no                                                                           & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Modeling \\ control flow\end{tabular}}             & yes                                                                     & yes                                                                          & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Modeling \\ meta-features flow\end{tabular}}       & no                                                                      & no                                                                           & no                  & yes            & no            & no            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Validation\\ data flow\end{tabular}}               & yes                                                                     & no                                                                           & no                & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Validation\\ control flow\end{tabular}}            & yes                                                                     & yes                                                                          & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Validating\\ meta-features flow\end{tabular}}      & no                                                                      & no                                                                           & no                  & no             & no            & no            \\ \hline
\end{tabular}





\caption {Comparison of the pipeline modelling methods using the nine selected criteria. It is possible for function composition, directed acyclic graphs and Petri nets to generate pipelines consisting of different component types, however, the execution of these component types is not supported by libraries by default. Therefore, the criterion of the three approaches is abstract.}
\label{tab:modeling_compare}
\vspace{-0.5cm}
\end{table}

==> tables/table_tools_features.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering


\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Tool}}                                 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Pipeline composition\\ or algorithm selection\end{tabular}}} & \multicolumn{5}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Hyperparameter\\ optimisation\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Programming\\ language\end{tabular}}} & \multirow{2}{*}{\textbf{Libraries}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Distributed\\ processing\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Auto\\ deployment\end{tabular}}} \\ \cline{3-7}
                                                               &                                                                                                                 & \textbf{a}         & \textbf{b}         & \textbf{c}        & \textbf{d}        & \textbf{e}        &                                                                                          &                                     &                                                                                            &                                                                                     \\ \hline
Auto-Weka 0.5                                                  & algorithm selection                                                                                             & yes                & -                  & -                 & yes               & -                 & Java, Python                                                                             & Weka                                & no                                                                                         & no                                                                                  \\ \hline
Auto-Weka 2.0                                                  & algorithm selection                                                                                             & yes                & -                  & -                 & -                 & -                 & Java, Python                                                                             & Weka                                & no                                                                                         & no                                                                                  \\ \hline
\begin{tabular}[c]{@{}l@{}}Auto-Weka \\ for MCPS\end{tabular}  & pipeline composition                                                                                            & yes                & -                  & -                 & yes               & -                 & Java, Python                                                                             & Weka                                & no                                                                                         & no                                                                                  \\ \hline
Auto-sklearn                                                   & pipeline composition                                                                                            & yes                & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
H20                                                            & algorithm selection                                                                                             & -                  & yes                & -                 & -                 & -                 & Java, Python                                                                             & -                                   & yes                                                                                        & no                                                                                  \\ \hline
TPOT                                                           & pipeline composition                                                                                            & -                  & -                  & yes               & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
Mathematica                                                    & algorithm selection                                                                                             & yes                & -                  & -                 & -                 & -                 & -                                                                                        & -                                   & no                                                                                         & no                                                                                  \\ \hline
MLBox                                                          & pipeline composition                                                                                            & yes                & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
Auto\_ml                                                       & pipeline composition                                                                                            & -                  & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
RapidMiner                                                     & pipeline composition                                                                                            & -                  & yes                & yes               & -                 & -                 & -                                                                                        & -                                   & yes                                                                                        & yes                                                                                 \\ \hline
ATM                                                            & pipeline composition                                                                                            & yes                & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & yes                                                                                        & no                                                                                  \\ \hline
\begin{tabular}[c]{@{}l@{}}AWS Machine\\ Learning\end{tabular} & algorithm selection                                                                                             & -                  & -                  & -                 & -                 & yes               & -                                                                                        & -                                   & yes                                                                                        & yes                                                                                 \\ \hline
\end{tabular}


\caption {Compare AutoML tools in term of (1) Ability to automatically construct pipelines or select algorithm, (2) Hyperparameter optimisation method (a. Bayesian optimisation, b. Grid search, c. Genetic algorithm, d. Random search, e. Others), (3) Programming language, (4) Libraries used for preprocessing, classification, regression and ensemble algorithms, (5) Ability to run on distributed environment, (6) Auto deploy predictive model/pipeline and generate APIs for end users. An AutoML tool can automatically construct and optimise a pipeline including at least two components is marked as \textit{pipeline composition}, and only automatically select an algorithm and optimise its hyperparameters is marked as \textit{algorithm selection}. Symbol '-' represents for not available information.   }
\label{tab:tool_compare}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_tpot_experiments.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering


\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
                                   &                        & \textbf{seed=0}    & \textbf{seed=1}                                                                      & \textbf{seed=2}   & \textbf{seed=3}   & \textbf{seed=4}    \\ \hline
\multirow{3}{*}{\textbf{abalone}}  & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{amazon}}   & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{car}}      & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{convex}}   & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & RandomForest       & RandomForest                                                                         & RandomForest      & XGBoost           & GradientBoosting   \\ \cline{2-7} 
                                   & \textbf{accuracy}      & 74.14              & {\ul 73.78}                                                                          & 74.97             & \textbf{78.89}    & 78.23              \\ \hline
\multirow{3}{*}{\textbf{dexter}}   & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & MultinomialNB                                                                        & MultinomialNB     & MultinomialNB     & MultinomialNB      \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & {\ul 92.78}                                                                          & \textbf{93.33}    & \textbf{93.33}    & \textbf{93.33}     \\ \hline
\multirow{3}{*}{\textbf{dorothea}} & \textbf{preprocessors} & -                  & -                                                                                    &                   & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & RandomForest                                                                         & DecisionTree      & -                 & RandomForest       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & \textbf{95.36}                                                                       & {\ul 94.78}       & -                 & \textbf{95.36}     \\ \hline
\multirow{3}{*}{\textbf{gcredit}}  & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{gisette}}  & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & LogisticRegression & -                                                                                    & -                 & -                 & LogisticRegression \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{97.29}     & -                                                                                    & -                 & -                 & {\ul 97.19}        \\ \hline
\multirow{3}{*}{\textbf{shuttle}}  & \textbf{preprocessors} & ZeroCount          & -                                                                                    & -                 & SelectPercentile  & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & XGBoost            & ExtraTrees                                                                           & RandomForest      & RandomForest      & GradientBoosting   \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{99.99}     & \textbf{99.99}                                                                       & \textbf{99.99}    & \textbf{99.99}    & \textbf{99.99}     \\ \hline
\multirow{3}{*}{\textbf{wineqw}}   & \textbf{preprocessors} & PolynomialFeatures & \begin{tabular}[c]{@{}l@{}}VarianceThreshold $\rightarrow$\\ StackingEstimator\end{tabular} & StackingEstimator & StackingEstimator & PolynomialFeatures \\ \cline{2-7} 
                                   & \textbf{predictor}     & ExtraTrees         & RandomForest                                                                         & ExtraTrees        & GradientBoosting  & ExtraTrees         \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{64.26}     & 58.13                                                                                & 62.70             & 58.00             & {\ul 58.07}        \\ \hline
\end{tabular}

\caption {Pipeline structure and accuracy in percentage generated by TPOT using different datasets and seed numbers}
\label{tab:tpot_exp}
\vspace{-0.5cm}
\end{table*}


\end{landscape}
